Axial phono-magnetic effects

Axial or circularly polarized phonons are collective lattice vibrations with angular momentum. Over the past decade they have emerged as a promising mechanism for the manipulation of magnetism, in parallel to well established optical protocols. In particular, coherent axial phonons were shown to induce magnetization in materials without spin-ordering, making them a viable tool for ultrafast magnetic switching. The experimental evidence suggests that the size of this magnetization is significant, opening a new research area on the phono-magnetic effect. Remarkably, the coupling of axial phonons to magnetism has been observed a broad class of materials, pointing to a universal nature of the underlying mechanisms. In this review article, we present the recent progress in the field. We give an introduction to the phenomenological perspective and an overview of the experimental evidence for the magnetization emerging from axial phonons, which includes discussing the observations of phonon Zeeman effect, the magneto-optical Kerr effect and the proximity-induced magnetization switching. We present recently proposed microscopic theories for the phono-magnetic effects, based on perturbation theory, adiabatic motion and Floquet theory as well as the emergence of the phonon magnetic moment due to artificial gauge fields or inertial effects. This summary allows us to see correspondences between the seemingly different theoretical approaches, facilitating a more complete perspective of the effect.

==> figures/Colors_Chalmers.tex <==

\definecolor{morkkoppar}{RGB}{0, 108, 92}  % dark petrol
\definecolor{koppar}{RGB}{0, 169, 157}   % petrol
\definecolor{lov}{RGB}{127, 181, 57}  % green
\definecolor{granit}{RGB}{93, 111, 122}  % gray
\definecolor{himmel}{RGB}{88, 176, 227} % light blue

\definecolor{kaffe}{RGB}{72, 55, 41} % brown 
\definecolor{tegel}{RGB}{241, 90, 34} % orange
\definecolor{energi}{RGB}{255, 203, 5} % yellow
\definecolor{vastkust}{RGB}{0, 48, 80} % dark blue
\definecolor{skymning}{RGB}{39, 0, 137} % purple/blue


\colorlet{cl1}{himmel}
\colorlet{cl2}{lov}
\colorlet{cl3}{tegel}
\colorlet{cl4}{energi}
\colorlet{cl5}{skymning}
\colorlet{cl6}{kaffe}
\colorlet{cl7}{vastkust}


\colorlet{dcl1}{vastkust}
\colorlet{dcl2}{tegel}
\colorlet{dcl3}{morkkoppar}
\colorlet{dcl4}{skymning}
\colorlet{dcl5}{energi}


